Deterministic Autopoietic Automata

This paper studies two issues related to the paper on Computing by Self-reproduction: Autopoietic Automata by Jiri Wiedermann. It is shown that all results presented there extend to deterministic computations. In particular, nondeterminism is not needed for a lineage to generate all autopoietic automata.

==> eptcsdata.tex <==
\providecommand{\event}{S. Barry Cooper \& Vincent Danos (eds.): Fifth Workshop on\\
Developments in Computational Models---Computational Models From Nature}
\providecommand{\volume}{9}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{49}
\providecommand{\eid}{6}

